Structural Causality-based Generalizable Concept Discovery Models

The rising need for explainable deep neural network architectures has utilized semantic concepts as explainable units. Several approaches utilizing disentangled representation learning estimate the generative factors and utilize them as concepts for explaining DNNs. However, even though the generative factors for a dataset remain fixed, concepts are not fixed entities and vary based on downstream tasks. In this paper, we propose a disentanglement mechanism utilizing a variational autoencoder (VAE) for learning mutually independent generative factors for a given dataset and subsequently learning task-specific concepts using a structural causal model (SCM). Our method assumes generative factors and concepts to form a bipartite graph, with directed causal edges from generative factors to concepts. Experiments are conducted on datasets with known generative factors: D-sprites and Shapes3D. On specific downstream tasks, our proposed method successfully learns task-specific concepts which are explained well by the causal edges from the generative factors. Lastly, separate from current causal concept discovery methods, our methodology is generalizable to an arbitrary number of concepts and flexible to any downstream tasks.

==> images/AnonymousSubmission/LaTeX/conclusion.tex <==
\section{Conclusion}
In this paper, we propose a novel methodology for causal concept discovery using disentangled representations of underlying generative factors. Our method is successful in identifying the causal relationships between the generative factors and the concepts specific to downstream tasks. Experiments performed on carefully curated downstream classification tasks sampled from datasets where the generative factors are well-defined demonstrate that our proposed method discovers correct causal relationships between generative factors and concepts. Our work opens doors for future research which unifies disentanglement and causal discovery of concepts.

==> images/AnonymousSubmission/LaTeX/experimental.tex <==
\section{Experiments}
\subsection{Dataset Descriptions}
\begin{itemize}    
\item \textbf{D-Sprites} \cite{dsprites17}: D-Sprites consists of procedurally generated samples from 6 independent generative factors. 
% These factors include - shape of the object, color (both categorical) and X,Y positions and orientations (integer values). 
Each object in the dataset is generated based on two categorical factors (shape, color) and four numerical factors (X position, Y position, orientation, scale).
The 6 factors are independent of each other. The dataset consists of 737280 images. 
% We utilize 70\% of the data for training the VAE and extracting concepts and 30\% for testing. 
\item \textbf{Shapes3D} \cite{3dshapes18}: Shapes3D dataset consists of synthetically generated samples from 6 independent generative factors consisting of color (hue) of floor, wall, object (float values) and scale, shape, and orientation in space (integer values). The dataset consists of 480000 images. 
% We utilize 70\% of the data for training the VAE and extracting concepts and 30\% for testing. 

    
\end{itemize}
\noindent \textbf{Split descriptions:} 
For each dataset, we utilize 70\% of the data for training the VAE and learning task-specific concepts and 30\% for testing. 
Due to the fact that every attribute value combination is present exactly once in the dataset - random splitting can make the sets imbalanced with respect to a particular attribute. We split the sets in 70/30 proportion of the shape, posX and posY attributes for the D-sprites dataset while considering floor, wall, object hue and shape for the Shapes3D dataset.

    \subsection{Task Descriptions}
We construct downstream tasks using combinations of generative factors. For each task, we consider $n\in\{2,3\}$ generative factors on random. A task is defined as having the label ``$1$'' when all factors satisfy a pre-defined criterion and having the label ``0'' in other cases. For categorical factors, we consider the presence of the exact values as boolean Truth, while for continuous factors we use a threshold to decide the boolean Truth value. For instance, for the d-Sprites dataset task in Figure~\ref{fig:motivation}, we adjudge the label 1 when `X-position' is less than $0.5$ and the `shape' value is exactly the categorical value ``heart''. We ignore tasks that impute a very small training set. The number and description of the generative factors is given in Table~\ref{tab:task-desc} along with the number of tasks considered in our experiments. Further details on task construction can be found in the Appendix.

\begin{table}[h]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccc}
\hline
Dataset   & \# of Factors & Description & \# of Tasks \\
\hline
\multirow{3}{*}{D-Sprites} &         \multirow{3}{*}{6}           &  Shape, Color,        &     \multirow{3}{*}{9}        \\
&                  & PosX, PosY, &  \\  
&                  &  Orient, Scale &  \\  
\hline
\multirow{2}{*}{Shapes 3D} &         \multirow{2}{*}{6}          &     floor, wall, object hue, & \multirow{2}{*}{12} \\
 &                   & scale, shape, orientation      &            \\
\hline
\end{tabular}}
\caption{Dataset generative factors description and the associated task statistics.}
\label{tab:task-desc}
\end{table}





\subsection{Architecture Overview}
\noindent \textbf{Variational autoencoder}: For the d-Sprites dataset, we utilize an encoder architecture consisting of 3 fully connected linear layers $[900,600,300]$. The input images are scaled to (96, 96). The activation function utilized is the Exponential Linear Unit (ELU). The latent dimension ($z_{dim}$) is kept as 16. The corresponding decoder consists of 4 fully connected linear layers [300, 300, 1024, 96*96]. 

For the Shapes3D dataset, the input images also contain color information. We utilize a convolutional encoder with 6 layers with [3, 32, 64, 64, 64, 16] channels each and $z_{dim}$ = 16. The decoder consists of 3 transpose convolutional layers [64, 64, 3]. The activation function used is ReLU.



\noindent \textbf{Concept learning framework}.
The number of generative factors $m$ is already known. For all our experiments, we keep the number of concepts the same as generative factors, i.e., $n=m$. Hence the shape of the transformation matrix $\mathbf{A}$ is $(n,n)$. We initialize the weight matrix as a unit vector $\mathbf{W} = \mathbf{1}_n$.

\subsection{Hyperparameter Settings}
The proposed framework is sensitive to two sets of hyperparameters, which control the VAE reconstruction and the concept learning, respectively. For d-Sprites, we utilize $\beta_1$ and $\beta_2$ as 1.0 and 0.6, while for the Shapes3D dataset, $\beta_1$ and $\beta_2$ are set as 0.8 and 0.8. The values of $\alpha$ and $\gamma$ are set to 0.5 for both datasets and $\delta$ is set as 0.5 and 0.8 respectively for d-Sprites and Shapes3D. In our experiments, we observe that Shapes3D is much more sensitive to hyperparameters. One possible cause for this behavior is the encoding of colors in concepts making them unstable.
The learning rate for the VAE is set as 1e-3 with a linear warmup. The number of epochs used to train the end-to-end system is 50. However, in the first 10 epochs, the matrix $\mathbf{A}$ and $\mathbf{W}$ are not tuned, as we intend to ensure that VAE learns to disentangle the generative factors first and then guide concept learning.

\subsection{Evaluation}
Our evaluation framework evaluates the proposed method using its most important objectives. The methodology of evaluation is detailed as follows:
\begin{itemize}
    \item \textbf{Disentangled latent representation learning performance:} The most important component of the proposed method is learning independent generative factors. Most disentanglement methodologies utilize the Maximal Information Coefficient (MIC) for estimating the degree of information relevance between the known (true) distribution and the learned distribution.
    \item \textbf{Task performance: } As we only consider binary downstream tasks for estimating concepts, we utilize accuracy as the metric and evaluate our approach on the test set. 
    \item \textbf{Causal matrix learning:} The causal matrix learned is characterized by the relative weights of the transitions. Hence, we evaluate how accurately the relevant factors are identified (true positives). We also calculate the number of wrongly weighted causal edges from irrelevant generative factors (false positives) and the missed edges from relevant factors (false negatives). 
    
\end{itemize}






==> images/AnonymousSubmission/LaTeX/introduction.tex <==
\section{Introduction}
The increasing proliferation of Deep Neural Networks (DNNs) has revolutionized multiple diverse fields of research such as vision, speech, and language \cite{he2016deep,vaswani2017attention}. Due to the black-box nature of DNNs, explaining DNN predictions is an active field of research that attempts to impart transparency and trustworthiness in their decision-making processes. Recent research has consolidated explainability into increasing levels of complexity. The most granular approaches attempt to assign importance scores to the raw features extracted from the data, while less granular approaches assign importance scores to data points (sets of features). Explaining DNNs using concepts is the highest level of abstraction, as concepts are high-level independent abstract entities shared among multiple similar data points that align with human understanding of the task at hand. However, the concepts learned by the models may be entangled with each other and are not identifiable with human-understandable semantics.

A parallel field of research - disentanglement representation learning \cite{bengio2013representation,higgins2018beta,kim2018disentangling,chen2018isolating} attempts to learn a lower-dimensional representation of data where each dimension independently represents a distinct property of the data distribution. These approaches attempt to mimic the underlying generation process of data, with the added goal of controlling and intervening to influence the generative process as well. These approaches learn mutually independent generative factors (usually called latents) by estimating their probability distribution from observed data. Once the probability distribution of the latents is inferred, the exact sample can be theoretically decomposed and generated from just its latents. For this reason, disentanglement approaches are considered to be explaining the generative process of data distribution - making them potentially highly interpretable. 

Though disentanglement representation learning makes it possible for the model to learn independent generative factors from data, it is not practical in real applications since the human-understandable concepts used in real-world tasks are usually related or even casually related to each other. Thus, another approach has been proposed to understand disentanglement using the lens of causality \cite{yang2021causalvae}. The motivation behind this approach is the assumption that disentangled latent representation act as endogenous causal variables for the data generation process. Causal representation learning attempts to incorporate and enforce graphical structure among the learned latent representation and assumes that the data generation process can be fully explained by transitions along graph edges. 
The task at hand then becomes simply to estimate the causal graph mapping from latent representations (endogenous) to the observed data (exogenous).


It is tempting to consider disentangled generative factors as concepts for explaining DNNs as generative factors are shared among all data points and are by definition independent. However, this line of thinking suffers from two distinct problems. The first problem relates to the fact that concepts used for explaining a specific DNN should be \textbf{task-specific}. For example, consider the example in Figure~\ref{fig:motivation} which attempts to infer understandable concepts for an image based on a particular ``task''. The image in question has been sampled from the d-Sprites \cite{dsprites17} dataset. The actor in question is interested in finding if the image contains a heart on the left of the center side of the image. Let us assume that the 1st concept encodes the shape and x-coordinate (position) of the image object. Now, we know that the shape and x-position are the only 2 factors that are responsible for making the task decision. Any other factors such as orientation, y-position, color, etc. are irrelevant to the task at hand. Now, let us assume that the task is switched to identifying if the heart is in the top half of the image. The generative factors remain the same, but the concepts change depending on the task, where now the concept encodes the shape and y-coordinate (position) of the image object. Hence, the goal is to encode relevant generative factors into concepts, not directly using generative factors as concepts. 



The second problem relates to the \textbf{non-identifiability} of generative factors in an unsupervised setting. This problem is well studied in disentanglement literature \cite{locatello2019challenging,locatello2020disentangling}.  Let us assume in Figure~\ref{fig:motivation} that the generative factors are not known at all and need to be inferred from just the observed data and the task at hand. Concepts can encode multiple generative factors and are by definition abstract entities. For datasets with added complexity, the generative factors do not correspond to the actual meaningful and helpful cues, but a combination of their encoding in concepts makes for easy human understanding.

Hence, the problem of learning task-specific concepts requires a task-guided concept learning framework, incorporating disentanglement approaches for learning the generative factors. Specifically, this paper:
\begin{itemize}
    \item Proposes a variational autoencoder-based model for learning disentangled generative factors, 
    \item Designs a structural causal model for mapping generative factors to task-specific concepts,
    \item Proposes a task structure to evaluate the flexibility and efficacy of the proposed framework, and  
    \item Utilizes datasets with known generative factors to evaluate the quality of generative factors encoded in concepts. 
\end{itemize}




\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{AnonymousSubmission/LaTeX/images/motivation-scm-causal.pdf}
    \caption{BOTTOM LEFT: Target image in question. Schematic figure to demonstrate why task-specific concepts are required. Even though the generative factors are known for the image, the concepts pertinent for correct classification can be causally related to multiple generative factors.}
    \label{fig:motivation}
\end{figure}


==> images/AnonymousSubmission/LaTeX/method.tex <==
\section{Methodology}
In this section, we first introduce the formulation of the structural causal model (SCM), which is designed to learn task-specific concepts. Next, we 
provide the procedure to learn disentangled representations using a variational autoencoder with the incorporation of our proposed SCM. Finally, we discuss the end-to-end training procedure followed by the final optimization objective. The schematic overview of our approach is presented in Figure~\ref{fig:schematic-figure}.  

% adding the notation for f,a,g
% Before detailing the formulation of the proposed approach, we first go over the definition and nomenclature of the variables. We start with exogenous variables, i.e., variables that can be observed and are provided as inputs for the training procedure. $X=\{\mathbf{x}\}$ and $U=\{\mathbf{u}\}$ represent training samples from a particular data distribution and associated labels of the underlying generative factors. The endogenous variables $\mathbf{Z=\{z}\}$ and $\mathbf{C=\{c\}}$ represent the associated latent representations and the causally learned task-specific concepts, respectively. $\mathbf{\epsilon}$ denotes the external independent noise variable in the process of data generation.

\subsection{Learning Concepts using Structural Causal Model}

\subsubsection{Transforming endogenous latent representations.}
Assume a set $Z= \{z_j\}_{j=1}^m$ consists of a mutually independent disentangled latent representation of generative factors of some data distribution, which is represented by a $m$-dimensional vector $\mathbf{z}$. Let ${C=\{c_i\}_{i=1}^n}$ denote a set of concepts describing some downstream task, represented by a vector $\mathbf{c}$ of size $n$. We propose to learn a causal representation of these task-specific concepts $\mathbf{c}$ based on the parent $\mathbf{z}$. Mathematically, we learn a structural causal model with $\mathbf{z}$ as independent parent nodes while concepts $\mathbf{c}$ are child nodes. The sets $Z$ and $C$ are ensured to be independent of each other and hence form a bipartite graph with directed edges from the set $Z$ to $C$. Mathematically we represent this procedure by 
\begin{equation}\label{eq:Z-to-C}
    \mathbf{c} = {h}(\mathbf{A}^{T}\mathbf{z}) + \mathbf{\epsilon}, \mathbf{\epsilon} \sim  \mathcal{N}(0,\,\mathbf{I}).
\end{equation}
In the equation, $\mathbf{A}$ denotes the causal matrix between the generative factors and concepts to be learned and $h$ corresponds to non-linear functions mapping transformed generative factors to concepts. $\mathbf{\epsilon}$ denotes the external independent noise multi-dimensional random variable in the process of data generation. The set of generative factors $Z$ and concepts $C$ form a bipartite graph $\Gamma$, implying no causal edges within $C$ or $Z$. In practice, we implement the transformation from $Z$ to $C$ as a linear layer. 
% Essentially, we optimize the following:
Specifically, each learnable concept $c_i$ is modeled as 

\begin{equation}
    \label{eq:z-to-c}
    {c_i} =  \mathbf{h}_i (\mathbf{A}_i\circ \mathbf{z};\eta_i) + \epsilon_i
\end{equation}
where $\mathbf{A}_i$ is a $m$-dimensional vector in $\mathbf{A} = \left[\mathbf{A}_1|\cdots|\mathbf{A}_n\right]$. The symbol $\circ$ denotes the element-wise multiplication. $\mathbf{h}_i$ is the non-linear mapping from the generative factors to the concept $c_i$, which is part of $h$. $\eta_i$ represents the parameters of the mapping $\mathbf{h}_i$. $\epsilon_i$ is a noise sampled from the standard Gaussian distribution $\mathcal{N}(0,1)$. The matrix $\mathbf{A}$ forms the core structural causal model (SCM) and models the graph edges between $Z$ and $C$ along with the functions $h$.

\subsubsection{Learning task-specific concepts.}
As postulated by \cite{koh2020concept}, concepts are independent and diverse entities that are utilized for downstream tasks. We propose to predict the downstream task label $y$ as a weighted sum of the concepts with bias. 
\begin{equation}
    y = \sigma(w_0 + \sum^n_{i=1} w_ic_i) ~or~   \mathbf{Y} = \mathbf{W^T}\mathbf{C}
\end{equation}
where $\{w_i\}_{i=1}^n$ are the estimated weights and $w_0$ is the bias. The function $\sigma$ is the logistic function that transforms the outputs into labels. 


\subsection{Learning Generative Disentangled Representations}
\subsubsection{Formulation of VAE.}
As the concepts $C$ are learned on the basis of the generative factors $Z$, an essential step of our proposed method is to learn mutually independent generative factors from the data. 
% We learn a disentangled representation $\mathbf{z}$ using parameters $\theta$ of the encoder $f$ by estimating the posterior distribution $p_{\theta}(z|x)$. 
We learn a disentangled representation $\mathbf{z}$ using parameters $\phi$ of the encoder $f$ by estimating the posterior distribution $q_{\phi}(z|x)$. 
The decoder $g$ of the VAE attempts to learn the details of the generative process of distribution $X$ conditioned on latent representation $z$, which is denoted by $p_{\theta^*}(x|z)$ where $\theta^*$ is the true parameter for the data generative process. 
With $x$ as the observed data and $\mathbf{u}$ as the labels of the generative factors $\mathbf{z}$, the probability distribution is parameterized by the endogenous variables $\mathbf{c,z}$ and exogenous variables $\mathbf{x,u,\epsilon}$.
\begin{equation}
    \mathbf{p_{\theta}(x,z,c,\epsilon|u) = \mathbf{p_{\theta}}(x|z,c,\epsilon,u)p_{\theta}(\epsilon,z,c|u)}
\end{equation}


\subsubsection{Noisy priors.}
Using the noisy inference strategy proposed in CausalVAE \cite{yang2021causalvae}, we can model the probability distribution $\mathbf{p_{\theta}(x|z,c,\epsilon,u)}$ with $\mathbf{p_{\theta}}(x|z,c)$ because the $\mathbf{\epsilon,u}$ do not affect the distribution of $\mathbf{x}$. 
It should be noted that estimating $\mathbf{p_{\theta}(x|z,c)}$ is equivalent to estimating $\mathbf{p_{\theta}(x|z)}$, since $\mathbf{c}$ can be modeled as a function of $\textbf{z}$ as mentioned in Equations \ref{eq:Z-to-C} and \ref{eq:z-to-c}. Hence
\begin{equation}
    \mathbf{p(c|x)} = \mathbf{p(h(z)|x)} \equiv \mathbf{p(z |x)} 
    \label{eq:c-independence}
\end{equation}

Mathematically, given an encoding function $f$ with parameters $\phi$ and a decoding function $g$ with parameters $\theta$, the reconstruction can be formulated on the latent representation $\mathbf{z}$:
\begin{equation}
    \mathbf{p_{\theta}(x|z,c) = p_{\xi}(x-g(z))}
\end{equation}
while the representations can be 
\begin{equation}
    \mathbf{q_{\phi}(z,c,\epsilon|x,u) = q(z,c|\epsilon)q_{\zeta}(\epsilon - f(x,u))} 
\end{equation}
The probability distributions of $\mathbf{p}$ and $\mathbf{q}$ are formulated using the encoder and decoder with differentiable functions $f$ and $g$, respectively, such that given the input image $x$ and associated labels $u$ for generative factors, the encoder and decoder formulations can be represented as follows.
\begin{equation}
    \mathbf{z} = \mathbf{f(\mathbf{x,u})}+\zeta ,~~ 
    \mathbf{x} = \mathbf{g(z)}+\xi
\end{equation}
where $\zeta$ and $\xi$ are noise variables sampled from distinct standard Gaussian distributions. 


% \subsubsection{Supervision using generative factor labels.}
% As the estimation of generative factors $Z$ is a completely unsupervised step, it suffers from the well-documented non-identifiability problem. In effect, this implies that the learned distribution $p(z|u)$ needs to be deterministic and grounded. As in \cite{yang2021causalvae}, we utilize a normal distribution with mean $\mathbf{u}$ and variance $1$.
% %%%%%% Still need more work on this

\begin{figure}
    \centering
    \includegraphics{AnonymousSubmission/LaTeX/images/Concept-Bipartite.pdf}
    \caption{Visualized graphical structure for mapping generative factors to task-specific concepts. The generated concepts are child terminal nodes of parent nodes corresponding to independent generative factors. The sets $Z \in\{z_i \}^N_1$ and $C \in\{c_i \}^K_1$  form a bipartite graph $\Gamma(Z,C)$ with directed edges from $Z$ to $C$. The edges from $Z$ to $C$ are modelled by the Causal Matrix $A$ which captures the edge transitions.}
    \label{fig:concept-bipartite}
\end{figure}

% \subsection{}

% \subsubsection{Learning task-specific concepts.}
% As postulated by \cite{}, concepts are independent and diverse entities which are utilized for dowstream task prediction. We propose to predict the dowstream task label $y$ as a weighted sum of the concepts with a bias term ($w_0$). 


% \begin{equation}
%     y = \sigma(w_0 + \Sigma^n_{i=1} w_ic_i) ~or~   \mathbf{Y} = \mathbf{W^T}\mathbf{C}
% \end{equation}
% where the function $\sigma$ is the logistic function which transforms the outputs into labels. 


\subsection{End-to-end Training}
\noindent \textbf{Estimating VAE parameters.} We utilize the Evidence Lower Bound (ELBO) criterion \cite{kingma2014auto} to estimate the probability distribution formulations in the VAE. Note that we have two sets of parameters in the encoder and decoder, parameterized by $\phi$ and $\theta$ respectively. We estimate the distribution $\mathbf{p_{\theta}(\epsilon,z,c|x,u)}$ by the corresponding ELBO formulations for VAEs \cite{kingma2014auto}.
\begin{align}
    \mathbb{E}_{q_\phi(\cdot|\mathbf{x})}[\log p_{\theta}(x|u)] \geq ELBO
\end{align}
% \begin{align}
%     \mathbb{E}_{q\mathbf{x}}[log p_{\theta}(x|u)] \geq ELBO
% \end{align}

The ELBO criterion can then be mathematically computed by ensuring conditioning on known distributions. Note that different from standard VAEs, we need to estimate both $\mathbf{z}$ and $\epsilon$ noise. Priors are introduced on $\epsilon$ using a pre-defined distribution. In our experiments, we utilize a standard normal distribution as prior for $\epsilon$, i.e., $p_{\epsilon}\sim \mathcal{N}(0,\mathbf{I})$. The ELBO criterion can be estimated as follows.
\begin{align*}
    \label{eq:elbo}
    ELBO = \mathbb{E}_{q} & [\mathbb{E}_{q_{\phi}(z,c|x,u)}[log ~p_{\theta}(x|z)]\\
    & - \beta_1\mathbb{D}_{KL}(q_{\phi}(\epsilon|x,u) || p_{\epsilon}(\epsilon)) \\
    & - \beta_2\mathbb{D}_{KL}(q_{\phi}(z,c|x,u) || p_{\theta}(z,c|u)) ]
\end{align*}
Note that $\mathbb{D}_{KL}(p|q)$ denotes the reverse KL-divergence between distributions $p$ and $q$. The strength of KL divergence in the ELBO criterion is controlled by 2 tunable hyperparameters - $\beta_1,$ and $\beta_2$.

\noindent \textbf{Supervision using generative factor labels $\mathbf{u}$.} To ensure the identifiability of disentangled latent variables, we provide supervision using generative factor labels. We minimize the effect of the transformation from $Z$ to $C$ by ensuring the inverse transform maps back to the identifiable labels.

\begin{equation}
    l_{u} = \mathbb{E}_{qx} \mathbf{ \|\sigma(u({A^{-1}c})) - \sigma(uz) \|^2_2 }  
\end{equation}

\subsubsection{Ensuring edge weight integrity.}
The causal matrix $\mathbf{A}$ maps the generative factors $Z$ to the concepts ${C}$. Due to the nature of SCM, the matrix $\mathbf{A}$ corresponds to a Directed Acyclic Graph. However, it is possible that during the training procedure, degnerate edge-weights are learned, due to imbalanced sampling of observed data. Hence, we utilize a regularization and thresholding procedure to ensure edge weight integrity.

For the regularization procedure, we ensure that there are no degenerate concepts among $C$, i.e., one concept does not dominate the causal graph. We regularize the matrix using Frobenius Norm which ensures that the entire matrix $\mathbf{A}$ does not assign 0 weight edges to the associated SCM.
\begin{equation}
    \label{eq:diversity}
    l_{{diversity}} = \|\mathbf{A}\|_F
\end{equation}

The goal of thresholding is to control the effect of a single matrix element (edge weight) dominating the causal graph, we clip the maximum and minimum values in the matrix $\mathbf{A}$ to $\{1,-1\}$ after normalization.
\begin{equation}
    \mathbf{A} = clip(\mathbf{A}\circ 1/max(\mathbf{||A||}),-1,1)
\end{equation}

\noindent \textbf{Task learning and concept diversity.} In our proposed approach, we evaluate only on binary tasks, however, without loss of generalizability, we can represent classification loss as with $N$ number of classes as:
\begin{equation}
    l_{clf} = -\sum^N_{i=1}y_i\log\hat{y}_i 
\end{equation}
In addition, we ensure concept diversity as mentioned in Equation~\ref{eq:diversity}.
The complete training objective with tunable hyperparameters $\alpha, \beta_1, \beta_2, \delta, \gamma$ is as follows. 
\begin{equation}
    \mathcal{L} = -ELBO (\beta_1,\beta_2) + \alpha l_u + \delta l_{clf} + \gamma l_{diversity}
    \label{eq:end2end}
\end{equation}
Note that $\beta_1$ and $\beta_2$ are hyperparameters controlling the effect of the KL divergence.  




==> images/AnonymousSubmission/LaTeX/relatedwork.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.7\textwidth]{AnonymousSubmission/LaTeX/images/ConceptSCM.pdf}
    \caption{Schematic diagram of the proposed approach to learn task-specific concepts from disentangled independent representations (generative factors). Our proposed approach utilizes a variational autoencoder to learn representations of mutually independent generative factors ($\mathbf{z}$). The generative factors are transformed into concepts $\mathbf{c}$ by the Structural Causal Matrix $\mathbf{A}$. Finally, task prediction is performed by the weighted sum of the concepts $c$ and Weight Matrix $W$. $\hat{x}$ represents the reconstructed $x$. The exact formulation is detailed in Appendix. \textit{Green} blocks represent exogenous variables, i.e., variables that can be observed and are provided as input to the model. \textit{Blue} blocks represent endogenous variables, i.e., variables learned from the model. \textit{Red} blocks represent learnable parameters of the model. (Best viewed in color)}
    \label{fig:schematic-figure}
    \vspace{-4pt}
\end{figure*}
\section{Related Work}

\subsection{Related work on Disentangled Representation Learning}

Disentangled representation learning has long been a fascinating study aimed at separating distinct informational factors of variations in real-world data \citep{bengio2013representation,locatello2019challenging}. 
Due to its probabilistic framework and flexibility to customize training objectives, the variational autoencoder (VAE) \citep{kingma2014auto} is a commonly used architecture in the study of disentangled representation learning, which can capture different factors of variation with its encoder and decoder. Based on the traditional VAE, \citet{higgins2018beta} proposed a variant, $\beta$-VAE, which introduces an additional hyperparameter to scale the importance of the regularization term. By changing the weight of the regularization term, $\beta$-VAE can control the trade-off between the reconstruction of inputs and the disentanglement of latent variables. Instead of optimizing the Kullback–Leibler (KL) divergence between the latent distribution and standard Gaussian prior for disentanglement as done by VAE and $\beta$-VAE, FactorVAE \citep{kim2018disentangling} and $\beta$-TCVAE \citep{chen2018isolating} further decompose the regularization term and propose to directly penalize the total correlation between latent variables, which are shown to better disentangle the variables.

While early studies in disentanglement representation learning attempted to learn independent latent variables by modifying the training objective of VAE \cite{higgins2018beta,kim2018disentangling,chen2018isolating}, \citet{locatello2019challenging} showed that it is impossible to learn disentangled latent variables without any supervision. A series of subsequent studies were then proposed to learn disentangled representations with better identifiability using different kinds of supervision \citep{locatello2020disentangling,shu2020weakly,shen2022weakly}.   


\subsection{Related work on Concept Based Explanations}

Due to the black-box nature of deep learning models, various approaches have been explored to provide explanations for the outcome of deep neural networks \citep{koh2020concept,pedapati2020learning,jeyakumar2020can,heskes2020causal,o2020generative}. One important direction is to interpret the models with intuitive and human-understandable concepts, which are usually high-level abstractions of the input features. Various attempts have been made to automatically learn the concepts for different tasks \citep{kim2018interpretability,ghorbani2019towards,yeh2020completeness,wu2020towards,goyal2019explaining}. Among them, the concept bottleneck model (CBM) \citep{koh2020concept} is a commonly used approach to incorporate the learning of concepts into deep neural networks. By constructing a low-dimensional intermediate layer in the models, CBMs are able to capture the high-level concepts that are related to the downstream tasks. Numerous studies have been carried out to adapt CBMs for tasks in various domains \citep{sawada2022concept,jeyakumar2021automatic,pittino2021hierarchical,bahadori2020debiasing}.

\subsection{Related work on Causality in Deep Learning and Structural Causal Models}

There are a series of works that incorporate structural causal models (SCMs) into the learning of generative models. CausalGAN \citep{kocaoglu2018causalgan} and CAN \citep{moraffah2020causal} are uni-directional generative models built on generative adversarial networks (GANs) \citep{goodfellow2014generative}, which assign SCMs to the conditional attributes while the latent variables are independent Gaussian noises. Since the ground-truth factors are directly fed into the generators in these two models as conditional attributes, they are not able to learn disentangled latent variables that are aligned with the factors. CausalVAE \citep{yang2021causalvae} and GraphVAE \citep{he2019variational} are two VAE-based models that involve SCMs during training. While CausalVAE directly assigns an SCM to the latent variables and adopts a conditional prior on them, GraphVAE imposes an SCM into the latent space of VAE by generalizing the chain-structured latent space proposed in LadderVAE \citep{sonderby2016ladder}, which is designed to improve expressive capacity of VAE.
\vspace{-2pt}



==> images/AnonymousSubmission/LaTeX/results.tex <==
\section{Results and Discussion}

\subsection{Quality of Latent Representation Learning}
We start by visualizing the reconstructions to provide a qualitative analysis of the training of the VAE. Figure~\ref{fig:reconstruction-vis} shows the reconstructed images randomly sampled from the test sets of d-Sprites and Shapes3D. It can be observed that our approach can well reconstruct the input images with the learned latent representations. Next, we report the MIC scores for both datasets in Table~\ref{tab:mic}. In the first and second rows (Row 1 and Row 2), we compare the scores with a  $\beta$-VAE without and with noisy inference. Row 3 reports the MIC scores of our proposed approach. We observe that the MIC scores for noisy inference $\beta$-VAEs (Row 5) with supervision labels are the highest, followed by standard $\beta$-VAEs (Row 4) with supervision. Our method is between noisy $\beta$-VAE and supervised $\beta$-VAE. This is expected, as we attempt to learn both concepts and latent representations together which causes the disentanglement performance to drop slightly.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{AnonymousSubmission/LaTeX/images/reconstructions-latents.pdf}
    \caption{TOP: Original test set images and their associated reconstructions from the d-Sprites dataset. BOTTOM: Original test set images and their associated reconstructions from the Shapes3D dataset. As can be seen, the reconstruction quality is perceptibly similar. }
    \label{fig:reconstruction-vis}
\end{figure}
\vspace{-10pt}
    \begin{table}[h]
    \centering
    \begin{tabular}{c|c||c}
    \hline
          & \textbf{D-Sprites} & \textbf{Shapes3D} \\
          \hline 
    $\beta$-VAE            &    0.48       &   0.41       \\
    Noisy $\beta$-VAE                           & 0.52          &  0.43         \\
    \textbf{Ours}                              & \textbf{0.77}          & \textbf{0.67}         \\
    Sup. $\beta$-VAE & 0.91          & 0.80         \\
    Sup. Noisy $\beta$-VAE                & 0.93          & 0.82       \\ 
    \hline
    \end{tabular}

\caption{MIC score values of our approach as compared to commonly utilized VAE formulations. Note that our approach also learns concepts along with disentangled latent representations.}
\label{tab:mic}
\end{table}

\vspace{-4pt}
\subsection{Effect of Classification Loss Weight $\delta$ on Accuracy and Disentanglement Performance}
We observe that the weight assigned to the classification loss is an extremely important hyperparameter. In Figure~\ref{fig:ablation-delta}, we show that a low $\delta$ results in higher MIC scores, but worse accuracy. On the other hand, with high $\delta$, we achieve very high accuracy but the MIC scores plummet implying a sensitive trade-off between task accuracy and disentanglement performance.


\begin{table}[h]
\begin{tabular}{c|cccc}
\hline
\textbf{D-Sprites} & \textbf{2-GF} & \textbf{3-GF} & \textbf{FP} & \textbf{FN} \\
\hline

Unconstrained         & 0.77             & 0.71             & 0.41                     & 0.26                     \\
w/ Thresholding        & 0.80             & 0.75             & 0.23                     & 0.17                     \\
\textbf{w/ Regularization}         & \textbf{0.93}             & \textbf{0.88}             & \textbf{0.13}                     & \textbf{0.09}                     \\
\hline
\textbf{Ground Truth}         &    0.99          &   0.97           &     0.01                &          0.02            \\

\hline

\end{tabular}
\\ 
\\
\\
\begin{tabular}{c|cccc}
\hline
\textbf{Shapes3D} & \textbf{2-GF} & \textbf{3-GF} & \textbf{FP} & \textbf{FN} \\
\hline
Unconstrained       &        0.44      &    0.41          &                 0.31    &            0.57         \\
w/ Thresholding        &     0.56        &    0.51          &         0.22             &           0.46          \\
\textbf{w/ Regularization}         &     \textbf{0.74}         &   \textbf{0.69}           &              \textbf{0.19}        &                \textbf{0.28}      \\
\hline
\textbf{Ground Truth}         &     0.93        &    0.93         &               0.01      &          0.07       \\
\hline
\end{tabular}
\caption{Performance of inferring the relevant and irrelevant generative factors for the learned causal  matrix $\mathbf{A}$ on the d-Sprites and Shapes3D datasets. The bottom-most row corresponds to the setting where the causal matrix is initialized based on ``known'' factor values. The first row denotes unconstrained $\mathbf{A}$, while second and third rows progressively add thresholding (clipping) and Frobenius regularization implying increasing constraints on learning $\mathbf{A}$.
}
\label{tab:dset-acc}
\vskip -15pt
\end{table}

\begin{figure*}[t]
    \centering
    \begin{subfigure}{.48\textwidth}
    \includegraphics[width=\textwidth]{AnonymousSubmission/LaTeX/images/CausalGraph-dsprites-t1.pdf}
    \caption{Learned task weights (left) and learned causal matrix $\mathbf{A}$\\ for the target binary task - ``heart shape \& left sided''. As can be \\ seen from the concept weights, concept ``C1'' causally encodes\\ information from ``shape'' and ``X-position'' and has the highest\\ edge weight during prediction.}
    \label{fig:dsprites-heatmap-t1}
    \end{subfigure}%
    \begin{subfigure}{.48\textwidth}
    \includegraphics[width=\textwidth]{AnonymousSubmission/LaTeX/images/CausalGraph-dsprites-t2.pdf}
    \subcaption{Learned task weights (left) and learned causal matrix $\mathbf{A}$ for the target binary task - ``Shape = heart \& position = top \& Scale $\geq 0.7$''. As can be seen from the concept weights, concept ``C6'' causally encodes information from ``Shape'', ``Scale'' and ``Y-position'' and has the highest edge weight during prediction.}
    \label{fig:dsprites-heatmap-t2}
    \end{subfigure}
    \caption{Visualizations of the learned edge weight matrices $\mathbf{W}$ and causal matrices $\mathbf{A}$ for 2 binary tasks for the d-Sprites dataset. Note that we plot the transpose of both matrices. The lighter the color, the higher the weight assigned to the edge is (Best viewed in color). Similar visualizations for the Shapes3D dataset can be found in Appendix.}
    \label{fig:dsprites-causal-analysis}
\end{figure*}


\subsubsection{Causal and weight matrix evaluation.}
\noindent Inferring the causal matrix is tricky because multiple causal edges from the generative factors to the concepts can be learned. In addition, it is impossible to control exactly which concept encodes the appropriate generative factors for a task. Hence, we infer the matrix in reverse - we observe the index of the highest weight in the weight matrix $\mathbf{W}$ - the most relevant concept for task performance. Subsequently, we observe the highest matrix entries associated with this particular concept which corresponds to the edge weights from the generative factors. We demonstrate the process visually in Figure~\ref{fig:dsprites-heatmap-t1}.

Figure~\ref{fig:dsprites-heatmap-t1} represents the weight and causal matrix $\mathbf{W}$ and $\mathbf{A}$ for the binary task constructed using ``Shape == Heart \& left sided == True''. We observe that the concept with the highest weight is ``C1'' and the causally associated generative factors ``shape'' and ``x-position'' are properly learned, represented by the highest relative entries along the ``C1'' concept column. Similarly, for Figure~\ref{fig:dsprites-heatmap-t2}, highest weighted concept ``C6'' encodes the 3 generative factors - ``shape'', ``scale'' and ``y-position''. We calculate the average correctly learned relevant generative factors for all tasks, non-learned relevant factors (false negatives-FN) as well as the wrongly learned irrelevant factors (false positives-FP) in Table~\ref{tab:dset-acc} for D-Sprites and Shapes3D datasets respectively. In the table, 2-GF and 3-GF represent tasks with 2 and 3 relevant generative factors (GFs) respectively. We also report the performances comparing the effect of thresholding and regularization (Rows 2 and 3). As expected, thresholding and regularization improve the accuracy of learning relevant and removing non-relevant generative factors. We also compare our performance to ground truth intialization where we initialize the causal matrix $\mathbf{A}$ with relevant generative factors and do not learn the causal matrix (Row 4).







\begin{figure}
    \centering
    \includegraphics[width=0.38\textwidth]{AnonymousSubmission/LaTeX/images/ablation-delta.png}
    \caption{The effect of $\delta$ on overall MIC values and average task accuracy. We observe a tradeoff between task accuracy and MIC values with increasing values of $\delta$.}
    \label{fig:ablation-delta}
\end{figure}







